For the Underrepresented in Gender Bias Research: Chinese Name Gender Prediction with Heterogeneous Graph Attention Network

Achieving gender equality is an important pillar for humankind's sustainable future. Pioneering data-driven gender bias research is based on large-scale public records such as scientific papers, patents, and company registrations, covering female researchers, inventors and entrepreneurs, and so on. Since gender information is often missing in relevant datasets, studies rely on tools to infer genders from names. However, available open-sourced Chinese gender-guessing tools are not yet suitable for scientific purposes, which may be partially responsible for female Chinese being underrepresented in mainstream gender bias research and affect their universality. Specifically, these tools focus on character-level information while overlooking the fact that the combinations of Chinese characters in multi-character names, as well as the components and pronunciations of characters, convey important messages. As a first effort, we design a Chinese Heterogeneous Graph Attention (CHGAT) model to capture the heterogeneity in component relationships and incorporate the pronunciations of characters. Our model largely surpasses current tools and also outperforms the state-of-the-art algorithm. Last but not least, the most popular Chinese name-gender dataset is single-character based with far less female coverage from an unreliable source, naturally hindering relevant studies. We open-source a more balanced multi-character dataset from an official source together with our code, hoping to help future research promoting gender equality.

==> tables/AblationResults.tex <==
\begin{table}[htb]

\centering
\small
\begin{tabular}{c|c|c|c|c}

\hline
 & FGAT& variant\_1 & variant\_2 & our model \\
\hline
accuracy& 0.8010 & 0.8112  & 0.8071 & 0.8173 \\
\hline
\end{tabular}


\caption{Accuracy of FGAT, variant\_1, variant\_2, and our model trained and tested on \textbf{9,800 Names}.}
\label{tab:result3}
\end{table}

==> tables/CharacterFormationTypes.tex <==
\begin{table}[htb]
\small
\centering
\begin{spacing}{1.2}
\begin{tabular}{|c|c|c|c|}
\hline
Index & Structure Type            & Icon & Example \\ \hline
1     & left to right             & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/1.png}}}$    & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/1_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/1_2.png}}}$        \\  \hline
2     & left to middle and right  & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/2.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/2_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/2_2.png}}}$      \\  \hline
3     & above to below            & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/3.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/3_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/3_2.png}}}$      \\  \hline
4     & above to middle and below & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/4.png}}}$    &     $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/4_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/4_2.png}}}$     \\  \hline
5     & full surround             & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/5.png}}}$    &     $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/5_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/5_2.png}}}$     \\  \hline
6     & surround from above       & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/6.png}}}$    &     $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/6_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/6_2.png}}}$     \\  \hline
7     & surround from below       & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/7.png}}}$    &     $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/7_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/7_2.png}}}$     \\  \hline
8     & surround from left        & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/8.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/8_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/8_2.png}}}$      \\  \hline
9     & surround from upper left  & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/9.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/9_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/9_2.png}}}$      \\  \hline
10    & surround from upper right & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/10.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/10_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/10_2.png}}}$      \\  \hline
11    & surround from lower left  & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/11.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/11_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/11_2.png}}}$      \\  \hline
12    & integral                  & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/12.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/12_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/12_2.png}}}$      \\  \hline
13    & isosceles triangle layout & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/13.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/13_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/13_2.png}}}$      \\  \hline
14    & square layout             & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/14.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/14_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/14_2.png}}}$      \\  \hline
15    & multielement combination  & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/15.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/15_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/15_2.png}}}$      \\  \hline
16    & overlaid                  & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/16.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/16_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/16_2.png}}}$      \\  \hline
17    & multielement stacking     & $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/17.png}}}$    &    $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/17_1.png}}}$, $\vcenter{\hbox{\includegraphics[width=0.29cm]{pictures/17_2.png}}}$      \\  \hline
\end{tabular}
\end{spacing}
\caption{The list of Chinese characters' formation types. The first 11 structure type names follow their unicode names, while the last 6 have no formal names, so we describe their structural characteristics as best we can.}
\label{tab:structure}
\end{table}

==> tables/DatasetDescription.tex <==
% \begin{table*}[htb]
% \small
%   \centering
%     \begin{tabular}{lcccc}
%     \toprule
%     &\multicolumn{1}{c}{Records}&\multicolumn{1}{c}{Unique First Names}&\multicolumn{1}{c}{Male Records}&\multicolumn{1}{c}{Female Records}\\
% \hline

% Ngender&     32,067,566&      9,442&    21,280,545&      10,787,021\\

% Our Dataset&     58,393,173&      560,706&    30,794,006&      27,599,167\\

% 9,800 Names&     9,800&      6,972&    4,900&      4,900\\

% 25,856 Names&     25,856&      21,051&    12,928&      12,928\\

%     \bottomrule
%     \end{tabular}%
  
%     \caption{Statistics of the datasets. For the Ngender dataset, we count its unique characters as its unique first names, since it is a single-character dataset.}
%     \label{tab: dataset describtion}
% \end{table*}%

\begin{table}[!hbt]
\small
  \centering
  \scalebox{0.95}{
    \begin{tabular}{lccc}
    \toprule
    &\multicolumn{1}{c}{Records}&\multicolumn{1}{c}{Unique First Names}&\multicolumn{1}{c}{M-to-F\%}\\
\hline

Ngender&     32,067,566&      9,442&  197.28\\

Our Dataset&     58,393,173&      560,706&  111.58  \\

9,800 Names&     9,800&      6,972& 100.00 \\

25,856 Names&     25,856&      21,051& 100.00 \\

    \bottomrule
    \end{tabular}%
    }
    \caption{Statistics of the datasets. For the Ngender dataset, we count its unique characters as its unique first names, since it is a single-character dataset. Besides, we show the ratio of males to females for each dataset.}
    \label{tab: dataset describtion}
\end{table}%



==> tables/ExperimentResults.tex <==
\begin{table*}[htb]
\small
  \centering

    \begin{tabular}{cccccc}

    \toprule
\multirow{3}{*}{ \makecell{}}&\multirow{3}{*}{} &
\multicolumn{4}{c}{Testing Dataset} \\\cmidrule(lr){3-6}

  \makecell[c]{Training} & \makecell[c]{Method}  & \makecell[c]{9,800 Names}   & \makecell[c]{25,856 Names} & Ngender  & Ours  \\
    \midrule
\multirow{4}{*}{\makecell{Ours}}&Ngender&0.7066&0.7529&0.6636&0.8757\\
    &PBERT&0.8136&0.8081&0.7849&0.9309\\
    &FGAT&0.8139&0.8126&0.7854&0.9329\\
    &CHGAT&\textbf{0.8147}&\textbf{0.8186}&\textbf{0.7873}&\textbf{0.9362}\\
    \midrule
\multirow{4}{*}{\makecell{Ngender\\ }}&Ngender&0.6868&0.7518&0.6636&0.8476\\
    &PBERT&0.7541&0.7776&0.8010&0.9012\\
    &FGAT&0.7798&0.7977&0.8042&0.9148\\
    &CHGAT&\textbf{0.7897}&\textbf{0.8040}&\textbf{0.8054}&\textbf{0.9168}\\
    \bottomrule
    \end{tabular}%
  
    \caption{Experiment results of all models trained on the Ngender data and our data, and tested on four datasets.}
    \label{tab: Method result}%
\end{table*}%

% \begin{table*}[htb]
% \small
%   \centering

%     \begin{tabular}{cccccc}

%     \toprule
% \multirow{3}{*}{ \makecell{}}&\multirow{3}{*}{} &
% \multicolumn{4}{c}{Testing Dataset} \\\cmidrule(lr){3-6}

%   \makecell[c]{Training} & \makecell[c]{Method}  & \makecell[c]{9,800 Names}   & \makecell[c]{25,856 Names} & Ngender  & Ours  \\
%     \midrule
% \multirow{4}{*}{\makecell{Ours}}&Ngender&0.7387&0.7670&0.6636&0.8757\\
%     &PBERT&0.8506&0.8232&0.7849&0.9309\\
%     &FGAT&0.8508&0.8278&0.7854&0.9329\\
%     &CHGAT&\textbf{0.8517}&\textbf{0.8339}&\textbf{0.7873}&\textbf{0.9362}\\
%     \midrule
% \multirow{4}{*}{\makecell{Ngender\\ }}&Ngender&0.7180&0.7658&0.6636&0.8476\\
%     &PBERT&0.7884&0.7921&0.8010&0.9012\\
%     &FGAT&0.8152&0.8126&0.8042&0.9148\\
%     &CHGAT&\textbf{0.8256}&\textbf{0.8190}&\textbf{0.8054}&\textbf{0.9168}\\
%     \bottomrule
%     \end{tabular}%
  
%     \caption{Experiment results of all models trained on the Ngender data and our data, and tested on four datasets.}
%     \label{tab: Method result}%
% \end{table*}%
